ScanDP: Generalizable 3D Scanning with Diffusion Policy

Learning-based 3D Scanning plays a crucial role in enabling efficient and accurate scanning of target objects. However, recent reinforcement learning-based methods often require large-scale training data and still struggle to generalize to unseen object categories.In this work, we propose a data-efficient 3D scanning framework that uses Diffusion Policy to imitate human-like scanning strategies. To enhance robustness and generalization, we adopt the Occupancy Grid Mapping instead of direct point cloud processing, offering improved noise resilience and handling of diverse object geometries. We also introduce a hybrid approach combining a sphere-based space representation with a path optimization procedure that ensures path safety and scanning efficiency. This approach addresses limitations in conventional imitation learning, such as redundant or unpredictable behavior. We evaluate our method on diverse unseen objects in both shape and scale. Ours achieves higher coverage and shorter paths than baselines, while remaining robust to sensor noise. We further confirm practical feasibility and stable operation in real-world execution.

==> tables/coverage_fov.tex <==
\begin{table*}[h]
  \centering
  \small
  \caption{\textbf{Coverage [\%]}}
  \begin{tabular}{lccc}
    \toprule
    Camera
      & \begin{tabular}{c}
        L515 \\ ($70^\circ \times 43^\circ$)
      \end{tabular}
      & \begin{tabular}{c}
        D435 \\ ($87^\circ \times 58^\circ$)
      \end{tabular}
      & \begin{tabular}{c}
        D415 \\ ($65^\circ \times 40^\circ$)
      \end{tabular} \\
    \midrule
    3D Diffusion Policy & 58.36 & 60.89 & 61.97 \\
    \textbf{ScanDP} & \textbf{89.44} & \textbf{83.13} & \textbf{97.40} \\
    \bottomrule
  \end{tabular}
\end{table*}


==> tables/noise_gaussian.tex <==
\begin{table}[h]
  \centering
  \small
  \caption{\textbf{Coverage [\%] under noisy inputs (Gaussian Noise).}}
  \begin{tabular}{lccc}
    \toprule
    std
      & \begin{tabular}{c}
        0.01
      \end{tabular}
      & \begin{tabular}{c}
        0.1
      \end{tabular}
      & \begin{tabular}{c}
        1
      \end{tabular} \\
    \midrule
    3D Diffusion Policy & \textbf{98.73} & 70.22 & 70.06 \\
    \textbf{ScanDP} & 98.00 & \textbf{88.93} & \textbf{90.44} \\
    \bottomrule
  \end{tabular}
\end{table}
  


==> tables/path-length.tex <==
\begin{table*}[t]
  \centering
  \caption{\textbf{Comparisons Path Length until the coverage meets 0.95.}}
  \label{tab:result_path-length}
  \begin{tabular}{lrrrr}
    \toprule
    Policy & Bunny & Spot & Teapot & Armadillo \\
    \midrule
    Diffusion Policy & & & & \\
    3D Diffusion Policy & 20.23 & 15.380 & 18.52 & 10.87 \\
    3D Diffusion Policy$\ast$ & 19.80 & 16.62 & 16.66 & 18.06 \\
    Improved 3D Diffusion Policy & & & & \\
    \midrule
    \textbf{Ours (Conv3D)} & & & & \\
    \textbf{Ours (SparseConv)} & 23.22 & 21.39 & 22.65 & 23.99 \\
    \midrule
  \end{tabular}
  \vspace{-3mm}
\end{table*}

